Soft Robotic Dynamic In-Hand Pen Spinning

Dynamic in-hand manipulation remains a challenging task for soft robotic systems that have demonstrated advantages in safe compliant interactions but struggle with high-speed dynamic tasks. In this work, we present SWIFT, a system for learning dynamic tasks using a soft and compliant robotic hand. Unlike previous works that rely on simulation, quasi-static actions and precise object models, the proposed system learns to spin a pen through trial-and-error using only real-world data without requiring explicit prior knowledge of the pen's physical attributes. With self-labeled trials sampled from the real world, the system discovers the set of pen grasping and spinning primitive parameters that enables a soft hand to spin a pen robustly and reliably. After 130 sampled actions per object, SWIFT achieves 100% success rate across three pens with different weights and weight distributions, demonstrating the system's generalizability and robustness to changes in object properties. The results highlight the potential for soft robotic end-effectors to perform dynamic tasks including rapid in-hand manipulation. We also demonstrate that SWIFT generalizes to spinning items with different shapes and weights such as a brush and a screwdriver which we spin with 10/10 and 5/10 success rates respectively. Videos, data, and code are available at https://soft-spin.github.io.

==> 7_acknowledgements.tex <==
\section*{Acknowledgements}


==> 8_appdix.tex <==
\section{Appendix}
\YC{Chris suggest removing this appendix and move all the details to the website}
\subsection{Experiment hardware details}
In all experiments, we used an X-Arm Lite 6 robot paired with the MOE-hand. The hand's tendons were driven by Dynamixel XC330-288-T servos, powered by a 5V, 3A DC power supply. While this setup provided sufficient power for picking the pen from the fixture, during high-speed spin motions, some servos occasionally shut off due to current limitations. This behavior was particularly seen on finger m1 and m2. Finger m1 stays mostly stationary, while finger m2 usually bend in one direction due to the large movement it has to take. Despite this, the CMA-ES algorithm successfully generated feasible spin motions, even though the MOE-hand was not originally designed for high-speed tasks. It is possible to use a power supply with higher output current, but forcing the servos to move might also damage the internal components of the MOE-fingers.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.97\linewidth]{figs/moe_base.pdf}
    \caption{Visualization of the CAD design for base holder of the MOE-fingers. The fingers are attached through screws using the slots on the sides of the holder. The MOE-finger attachment configuration are marked on above the slots}
    \label{fig:MOE-Base}
\end{figure}

Fig.~\ref{fig:MOE-Base} illustrates the CAD design of the MOE-hand's base and the finger installation. The base is configured with the fingers angled inward, optimizing the grip for securely holding a pen. Slots on the sides of the base enable reconfiguration of the fingers as needed. Two slots were made on the side where the finger M1 was attached to, but only the center slot on that side was used in the experiments. 

Notably, finger M1 extends further forward than the other fingers, offering a larger surface area for the pen to stably spin around. Lastly, to reduce friction, a small piece of plastic tape is affixed to the back of finger M3, helping to minimize drag and prevent the pen from slowing down prematurely during spinning. 
\subsection{Hyperparemeters}
We initialize the CMA-ES generations using the following values [0,0,0.5,1.0,0.5,1.0,0.0,0.0]. The first six elements corresponds to the normalized $s_k'$, while $g_k'$ and $d_k'$ are both initialized to 0. For each of the 6 servos on the MOE-hand, we scale each element of $s_k'$ by [30,35,70,70,35,45] to get the final $s_k$ in degree angles for the servos to execute. The delay amount was scaled by $\lambda_d = 0.2$ and $\beta_d = 0.7$, so that the delay time is always limited to between $0.5$s and $0.9$s.  
% MOE finger motion limits
% MOE finger catch delay range
% % initialization
% bounding box 
% number of points threshold 
% number of frames per spin trial
% population size

Variations in the production quality of the MOE-fingers may require parameter adjustments in the CMA-ES algorithm to achieve successful spins. The parameter values we provide should be considered rough guidelines rather than definitive settings. Similarly, fine-tuning may be necessary for the robot arm carrying the MOE-hand to ensure optimal performance. Grasping and picking procedures might also require manual adjustments depending on the robot's configuration and the placement of fixtures. As such, we have not included exact joint or servo angles for achieving a stable grasp during spins. The grasping position can vary significantly based on the fixtures and pen's position relative to the robot arm, so exact values for grasping ranges are also not provided.



\subsection{Heuristics}
Color thresholding for pen tracking can fail under varying lighting conditions. To address this, we manually select key points on the first depth camera image. These points are then input into SAM v2, with no changes required for the rest of the state estimation pipeline. For experiments involving the brush and screwdriver, key points are similarly annotated by a human for SAM v2. While more advanced object tracking methods could be employed, optimizing this is beyond the scope of our current work and is left for future research.

Before each spin trial, the robot arm holds the MOE-hand at a slightly tilted but nearly horizontal angle. This positioning aids the spin by allowing gravity to assist in pulling the object around finger m1 after it has finished half a spin, reducing the acceleration needed for a full spin at the beginning. Additionally, the tilt helps prevent the object from falling off the front of the fingers by slightly guiding it toward the base of the MOE-hand, making it easier to for the MOE-hand to catch the object. For grasping, the MOE-fingers were adjusted to hold the object as close to the semi-hemispherical tips of the fingers as possible while still maintaining a secure grip until the spin configuration is reached. Grasping too far from the finger tips towards the black main bodies of the fingers increased the frequency of the object being caught by the fingers. This led to a very high number of failures and limited the CMA-ES algorithm’s ability to find effective spin motions.

==> extended_abstract.tex <==
\section{Introduction}






